Multi-Kernel Polar Codes: Concept and Design Principles

In this paper, we propose a new polar code construction by employing kernels of different sizes in the Kronecker product of the transformation matrix, thus generalizing the original construction by Arikan. The proposed multi-kernel polar code allows for more flexibility in terms of the code length, moreover allowing for various new design principles. We describe in detail encoding as well as successive cancellation (SC) decoding and SC list (SCL) decoding, and we provide a novel design method for the frozen set that allows to optimise the performance under list decoding, as opposed to original relability-based code design. Finally, we numerically demonstrate the advantage of multi-kernel polar codes under the new design principles compared to punctured and shortened polar codes.

==> figures/G_6.tex <==


\begin{figure}[h!]
\begin{center}
\resizebox{0.55\textwidth}{!}{\begin{tikzpicture}
[
	xscale	= 1,	% to scale horizontally everything but the text
	yscale	= 1,	% to scale vertically everything but the text
]



% ------------------------------------------------------
% NODES DEFINITION
\matrix
(nMatrix)
[
	row sep		= 0.6cm,
	column sep	= 2.1cm, ampersand replacement=\&
]
{


\node (n01) {$u_0$}; \&\node (n02)  {};\& [-4ex]\node (n03) {};\&\node (n04) {};\& [-4ex]\node (n05) {};\&\node (n06) {$x_0$};
	\\
\node (n11) {$u_1$};\&\node(n12) {};\&\node (n13) {};\&\node (n14) {};\&\node (n15) {};\&\node (n16) {$x_1$};\& \\

\node (n21) {$u_2$};\&\node(n22) {};\&\node(n23) {};\&\node (n24) {};\&\node (n25) {};\&\node (n26) {$x_2$};\\
% row 4
\node (n31) {$u_3$};\&\node(n32) {};\&\node(n33) {};\&\node(n34) {};\&\node (n35) {};\&\node (n36) {$x_3$};\\
% row 5
\node (n41) {$u_4$};\&\node(n42) {};\&\node(n43) {};\&\node(n44) {};\&\node(n45) {};\&\node (n46) {$x_4$};\&\\
% row 6
\node (n51) {$u_5$};\&\node (n52) {};\&\node(n53) {};\&\node(n54) {};\&\node(n55) {};\&\node(n56) {$x_5$};\&\\
};



%%% -------------------------
%% auxiliary nodes


\draw [LinesStyle] (n01) -- (n06) ;

\draw [LinesStyle] (n11) -- ($(n13.west) + (-.3cm,-0cm)$) ;
\draw [LinesStyle] ($(n13.west) + (-.3cm,-0cm)$) --  ($(n23.east) + (.3cm,-0cm)$);
\draw [LinesStyle] ($(n15.west) + (-.3cm,-0cm)$) -- ($(n13.east) + (.3cm,-0cm)$) ;
\draw [LinesStyle] ($(n15.west) + (-.3cm,-0cm)$) -- ($(n35.east) + (.3cm,-0cm)$) ;
\draw [LinesStyle] ($(n15.east) + (.3cm,-0cm)$) -- (n16) ;
%
\draw [LinesStyle] (n21) -- ($(n23.west) + (-.3cm,-0cm)$) ;
\draw [LinesStyle] ($(n23.west) + (-.3cm,-0cm)$) --  ($(n43.east) + (.3cm,-0cm)$);
\draw [LinesStyle] ($(n25.west) + (-.3cm,-0cm)$) -- ($(n23.east) + (.3cm,-0cm)$) ;
\draw [LinesStyle] ($(n25.west) + (-.3cm,-0cm)$) -- ($(n15.east) + (.3cm,-0cm)$) ;
\draw [LinesStyle] ($(n25.east) + (.3cm,-0cm)$) -- (n26) ;
%
\draw [LinesStyle] (n31) -- ($(n33.west) + (-.3cm,-0cm)$) ;
\draw [LinesStyle] ($(n33.west) + (-.3cm,-0cm)$) --  ($(n13.east) + (.3cm,-0cm)$);
\draw [LinesStyle] ($(n35.west) + (-.3cm,-0cm)$) -- ($(n33.east) + (.3cm,-0cm)$) ;
\draw [LinesStyle] ($(n35.west) + (-.3cm,-0cm)$) -- ($(n45.east) + (.3cm,-0cm)$) ;
\draw [LinesStyle] ($(n35.east) + (.3cm,-0cm)$) -- (n36) ;
%
\draw [LinesStyle] (n41) -- ($(n43.west) + (-.3cm,-0cm)$) ;
\draw [LinesStyle] ($(n43.west) + (-.3cm,-0cm)$) --  ($(n33.east) + (.3cm,-0cm)$);
\draw [LinesStyle] ($(n45.west) + (-.3cm,-0cm)$) -- ($(n43.east) + (.3cm,-0cm)$) ;
\draw [LinesStyle] ($(n45.west) + (-.3cm,-0cm)$) -- ($(n25.east) + (.3cm,-0cm)$) ;
\draw [LinesStyle] ($(n45.east) + (.3cm,-0cm)$) -- (n46) ;


\draw [LinesStyle] (n51) -- (n56) ;


\node [coordinate, xshift = -0.3cm, yshift =  0.3cm] (nAux1) at (n03.north west) {};
\node [coordinate, xshift =  0.3cm, yshift =  -0.3cm] (nAux2) at (n53.south east) {};
\draw [HighlightingStyle]  (nAux1) -| (nAux2) -|  (nAux1)
node [below, pos = 0.21] {};% {$P_2$};

\node [coordinate, xshift = -0.3cm, yshift =  0.3cm] (nAux3) at (n05.north west) {};
\node [coordinate, xshift =  0.3cm, yshift =  -0.3cm] (nAux4) at (n55.south east) {};
\draw [HighlightingStyle] (nAux3) -| (nAux4) -|  (nAux3)
node (Pnode) [below, pos = 0.21] {};% {$P_1$};

\node [coordinate, xshift = -0.3cm, yshift =  0.2cm] (nAux5) at (n02.north west) {};
\node [coordinate, xshift = 0.2cm, yshift =  -0.2cm] (nAux6) at (n22.south east) {};
\draw [HighlightingStyleB,fill=white] (nAux5) -| (nAux6) -|  (nAux5)
node (Pnode1) [xshift=0.4cm, yshift =-1.4cm] {$T_3$};

\node [coordinate, xshift = -0.3cm, yshift =  0.2cm] (nAux7) at (n32.north west) {};
\node [coordinate, xshift = 0.2cm, yshift =  -0.2cm] (nAux8) at (n52.south east) {};
\draw [HighlightingStyleB,fill=white] (nAux7) -| (nAux8) -|  (nAux7)
node (Pnode1) [xshift=0.4cm, yshift =-1.4cm] {$T_3$};

\node [coordinate, xshift = -0.3cm, yshift =  0.2cm] (nAux9) at (n04.north west) {};
\node [coordinate, xshift = 0.2cm, yshift =  -0.2cm] (nAux10) at (n14.south east) {};
\draw [HighlightingStyleB,fill=white] (nAux9) -| (nAux10) -|  (nAux9)
node (Pnode1) [xshift=0.4cm, yshift =-.9cm] {$T_2$};

\node [coordinate, xshift = -0.3cm, yshift =  0.2cm] (nAux11) at (n24.north west) {};
\node [coordinate, xshift = 0.2cm, yshift =  -0.2cm] (nAux12) at (n34.south east) {};
\draw [HighlightingStyleB,fill=white] (nAux11) -| (nAux12) -|  (nAux11)
node (Pnode1) [xshift=0.4cm, yshift =-.9cm] {$T_2$};

\node [coordinate, xshift = -0.3cm, yshift =  0.2cm] (nAux13) at (n44.north west) {};
\node [coordinate, xshift = 0.2cm, yshift =  -0.2cm] (nAux14) at (n54.south east) {};
\draw [HighlightingStyleB,fill=white] (nAux13) -| (nAux14) -|  (nAux13)
node (Pnode1) [xshift=0.4cm, yshift =-0.9cm] {$T_2$};

%\node[left of = n02,yshift=0.18cm,xshift=-0.05cm] (LLR20) {\footnotesize{LLR$(2,0)$}};
%\node[left of = n12,yshift=0.18cm,xshift=-0.05cm] (LLR21) {\footnotesize{LLR$(2,1)$}};
%\node[left of = n22,yshift=0.18cm,xshift=-0.05cm] (LLR22) {\footnotesize{LLR$(2,2)$}};
%\node[left of = n32,yshift=0.18cm,xshift=-0.05cm] (LLR23) {\footnotesize{LLR$(2,3)$}};
%\node[left of = n42,yshift=0.18cm,xshift=-0.05cm] (LLR24) {\footnotesize{LLR$(2,4)$}};
%\node[left of = n52,yshift=0.18cm,xshift=-0.05cm] (LLR25) {\footnotesize{LLR$(2,5)$}};
%
%\node[left of = n04,yshift=0.18cm,xshift=-0.05cm] (LLR10) {\footnotesize{LLR$(1,0)$}};
%\node[left of = n14,yshift=0.18cm,xshift=-0.05cm] (LLR11) {\footnotesize{LLR$(1,1)$}};
%\node[left of = n24,yshift=0.18cm,xshift=-0.05cm] (LLR12) {\footnotesize{LLR$(1,2)$}};
%\node[left of = n34,yshift=0.18cm,xshift=-0.05cm] (LLR13) {\footnotesize{LLR$(1,3)$}};
%\node[left of = n44,yshift=0.18cm,xshift=-0.05cm] (LLR14) {\footnotesize{LLR$(1,4)$}};
%\node[left of = n54,yshift=0.18cm,xshift=-0.05cm] (LLR15) {\footnotesize{LLR$(1,5)$}};
%
%\node[left of = n06,yshift=0.18cm,xshift=-0.05cm] (LLR00) {\footnotesize{LLR$(0,0)$}};
%\node[left of = n16,yshift=0.18cm,xshift=-0.05cm] (LLR01) {\footnotesize{LLR$(0,1)$}};
%\node[left of = n26,yshift=0.18cm,xshift=-0.05cm] (LLR02) {\footnotesize{LLR$(0,2)$}};
%\node[left of = n36,yshift=0.18cm,xshift=-0.05cm] (LLR03) {\footnotesize{LLR$(0,3)$}};
%\node[left of = n46,yshift=0.18cm,xshift=-0.05cm] (LLR04) {\footnotesize{LLR$(0,4)$}};
%\node[left of = n56,yshift=0.18cm,xshift=-0.05cm] (LLR05) {\footnotesize{LLR$(0,5)$}};

\node[left of = Pnode,node distance = 1.7cm] {Stage 1};
\node[left of = Pnode,node distance = 5.8cm] {Stage 2};
\end{tikzpicture}}
\caption{Tanner graph of the multi-kernel polar code for $G_6=T_2 \otimes T_3$.}
\label{fig:G_6}
%
\end{center}
\end{figure}
